Critical or Compliant? The Double-Edged Sword of Reasoning in Chain-of-Thought Explanations

Explanations are often promoted as tools for transparency, but they can also foster confirmation bias; users may assume reasoning is correct whenever outputs appear acceptable. We study this double-edged role of Chain-of-Thought (CoT) explanations in multimodal moral scenarios by systematically perturbing reasoning chains and manipulating delivery tones. Specifically, we analyze reasoning errors in vision language models (VLMs) and how they impact user trust and the ability to detect errors. Our findings reveal two key effects: (1) users often equate trust with outcome agreement, sustaining reliance even when reasoning is flawed, and (2) the confident tone suppresses error detection while maintaining reliance, showing that delivery styles can override correctness. These results highlight how CoT explanations can simultaneously clarify and mislead, underscoring the need for NLP systems to provide explanations that encourage scrutiny and critical thinking rather than blind trust. All code will be released publicly.

==> latex/figures/input_tex/rq1_result_figures.tex <==
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{latex/figures/01_detection_grouped_bar.png}
%     \vspace{4pt}
%     \includegraphics[width=0.8\linewidth]{latex/figures/02_agreement_grouped_bar.png}
%     \vspace{4pt}
%     \includegraphics[width=0.8\linewidth]{latex/figures/03_trust_grouped_bar.png}
%     % \caption{\textbf{Reliance outcomes.}
%     % (a) Grouped means of error detection rates by error type and correctness
%     % (b) Agreement with the model’s judgment.
%     % (c) Self-reported trust.}
%     \caption{\textbf{Reliance outcomes across error types.} 
% (a) Error detection,
% (b) agreement with the model’s moral judgment, and
% (c) self-reported trust in the model’s reasoning
% across error type and correctness. }
% % Detection increases when the final outcome is incorrect, yet omissions remain the least detectable. 
% % Agreement and trust both stay elevated for flawed but \textsc{Correct} judgments—especially omissions—revealing how plausible conclusions can mask reasoning flaws.}
%     \label{fig:measures_per_correctness}
% \end{figure}
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{latex/figures/figure3.pdf}
  \caption{\textbf{Reliance outcomes across error types.} 
(a) Error detection,
(b) agreement with the model’s moral judgment, and
(c) self-reported trust in the model’s reasoning
across error type and correctness.}
% Detection increases when the final outcome is incorrect, yet omissions remain the least detectable. 
% Agreement and trust both stay elevated for flawed but \textsc{Correct} judgments—especially omissions—revealing how plausible conclusions can mask reasoning flaws.}
    \label{fig:measures_per_correctness}
\end{figure}

==> latex/sections/app-roscoe-details.tex <==
 \subsection{Full ROSCOE diagnostic table}
  \label{app:roscoe-full}

  For completeness, Table~\ref{tab:roscoe-full} reports every ROSCOE metric we
  computed alongside the two verdict-link diagnostics introduced in the main
  text. The four columns of the main table
  (Tab.~\ref{tab:roscoe-selectivity}) are a curated subset of these eleven
  rows. We include the full set here to make three properties of the data
  inspectable: (i) the four reference-based metrics that saturate
  tautologically on clean chains and therefore require one-sample $d$ against
  the constant baseline of $1.0$; (ii) the cascading reference-coverage
  effects on Missing-Step that motivate our decision to report it as a
  diagnostic rather than as a perturbation-specific marker; and (iii) the
  under-firing of \textsc{Source-Consistency} (discourse representation) on
  \textsc{Hallucination}, which sits inside the clean-to-clean null band and
  which motivates the introduction of the verdict-link metrics.

  \begin{table*}[t]
  \centering
  \small
  \setlength{\tabcolsep}{6pt}
  \renewcommand{\arraystretch}{1.25}
  \begin{tabular}{l l c ccc}
  \toprule
  \textbf{Metric} & \textbf{Perspective} & \textbf{$d$ kind}
   & \textbf{\textsc{Omission}}
   & \textbf{\textsc{Contradiction}}
   & \textbf{\textsc{Hallucination}} \\
  \midrule
  \multicolumn{6}{l}{\textit{Semantic Alignment} (SBERT cosine between chain steps and source/reference)} \\
  \midrule
  Faithfulness                & SAL & paired
   & $-0.20\ {\scriptstyle[-0.40,+0.03]}$
   & $-0.12\ {\scriptstyle[-0.32,+0.11]}$
   & $-0.38\ {\scriptstyle[-0.61,-0.15]}$ \\
  Informativeness (step)      & SAL & paired
   & $+0.01\ {\scriptstyle[-0.22,+0.24]}$
   & $-0.16\ {\scriptstyle[-0.37,+0.07]}$
   & $-0.20\ {\scriptstyle[-0.45,+0.02]}$ \\
  Informativeness (chain)     & SAL & paired
   & $+0.22\ {\scriptstyle[-0.00,+0.42]}$
   & $+0.28\ {\scriptstyle[+0.10,+0.45]}$
   & $+0.49\ {\scriptstyle[+0.31,+0.70]}$ \\
  Missing-Step$^{\star}$      & SAL & 1-samp.
   & $\mathbf{+2.38}\ {\scriptstyle[+2.06,+2.88]}$
   & $+1.24\ {\scriptstyle[+1.09,+1.47]}$
   & $+1.53\ {\scriptstyle[+1.33,+1.82]}$ \\
  External Hallucination$^{\star}$ & SAL & 1-samp.
   & $+0.85\ {\scriptstyle[+0.73,+1.01]}$
   & $+1.13\ {\scriptstyle[+0.99,+1.35]}$
   & $+1.33\ {\scriptstyle[+1.17,+1.56]}$ \\
  Semantic Coverage (step)$^{\star}$  & SAL & 1-samp.
   & $+1.00\ {\scriptstyle[+0.87,+1.21]}$
   & $+0.73\ {\scriptstyle[+0.61,+0.92]}$
   & $+0.86\ {\scriptstyle[+0.74,+1.05]}$ \\
  Semantic Coverage (chain)$^{\star}$ & SAL & 1-samp.
   & $+0.67\ {\scriptstyle[+0.57,+1.00]}$
   & $+0.35\ {\scriptstyle[+0.28,+0.73]}$
   & $+0.82\ {\scriptstyle[+0.66,+1.25]}$ \\
  \midrule  
  \multicolumn{6}{l}{\textit{Logical Inference} (DeBERTa-v3 NLI; source- and self-consistency)} \\
  \midrule
  Source Consistency (Discourse Rep.)        & LI  & paired
   & $-0.46\ {\scriptstyle[-0.60,-0.32]}$
   & $+0.40\ {\scriptstyle[+0.20,+0.60]}$
   & $-0.06\ {\scriptstyle[-0.30,+0.16]}^{\,\ddagger}$ \\
  Self-Consistency (Coherence step-step)         & LI  & paired
   & $+0.03\ {\scriptstyle[-0.20,+0.27]}$
   & $\mathbf{+1.04}\ {\scriptstyle[+0.85,+1.29]}$
   & $+0.64\ {\scriptstyle[+0.46,+0.84]}$ \\
  \midrule  
  \multicolumn{6}{l}{\textit{Verdict-link} (NLI between chain premises and conclusion; this work)} \\
  \midrule
  Verdict Entailment          & VL  & paired
   & $+1.01\ {\scriptstyle[+0.81,+1.26]}$
   & $+0.74\ {\scriptstyle[+0.53,+0.96]}$
   & $\mathbf{+0.85}\ {\scriptstyle[+0.67,+1.07]}$ \\
  Verdict Contradiction$^{\dagger}$ & VL  & paired
   & $+0.47\ {\scriptstyle[+0.32,+0.62]}$
   & $+0.68\ {\scriptstyle[+0.46,+0.90]}$
   & $+0.76\ {\scriptstyle[+0.60,+0.95]}$ \\
  \bottomrule
  \end{tabular}
  \caption{\textbf{Full ROSCOE diagnostic table.} Signed Cohen's $d$ for
  the \textsc{Clean}$\rightarrow$perturbed shift on every metric we
  computed, with 95\% bootstrap CIs in brackets. All metrics oriented so that
  \emph{positive} $d$ denotes degradation. \textbf{Bold} marks the cells
  reported in the main diagnostic table (Tab.~\ref{tab:roscoe-selectivity}).
  $^{\star}$Reference-based metric: clean chains saturate at $1.0$ by
  construction, so we report one-sample $d$ against that constant baseline;
  all other rows use paired $d$ on matched triplets.
  $^{\ddagger}$Source-Consistency on \textsc{Hallucination} sits inside the
  clean-to-clean split-half null band ($|d|\le 0.46$); ROSCOE's text-only
  NLI formulation cannot detect visually-grounded fabrications when the
  source is a brief scenario prompt rather than an image description.
  $^{\dagger}$Verdict Contradiction is reverse-scored before computing $d$
  so that positive values share the same interpretation across columns.
  SAL = Semantic Alignment, LI = Logical Inference, VL = Verdict-link.}
  \label{tab:roscoe-full}
  \end{table*}
  
  \paragraph{Reading the full table.}
  Three patterns are visible in Table~\ref{tab:roscoe-full}. First, the
  three semantic-alignment metrics computed against the source
  (\textsc{Faithfulness}, \textsc{Informativeness}-step / chain) show
  small effects across all perturbation types ($|d|\!\lesssim\!0.5$):
  the Moralise source is thin and is not the locus of degradation for
  any of the perturbations we study. Second, the four reference-based
  metrics (marked $^{\star}$) all fire on every perturbation type, with
  \textsc{Missing-Step} fluctuating by perturbation in a way that does
  \emph{not} cleanly track the intended omission target ($d{=}2.38$ for
  omission but $d{=}1.53$ for hallucination and $d{=}1.24$ for
  contradiction). This is consistent with all three perturbations
  replacing or distorting clean reference content rather than only
  omission doing so; for that reason we frame \textsc{Missing-Step} as a
  generic reference-coverage diagnostic in the main table rather than as
  an omission-specific marker. Third, on \textsc{Hallucination}, ROSCOE's
  intended diagnostic metric --- \textsc{Source-Consistency} --- sits
  inside the clean-to-clean null band ($d{=}-0.06$, 95\% CI
  $[-0.30,+0.16]$). The verdict-link metrics we introduce
  (\textsc{Verdict Entailment} and \textsc{Verdict Contradiction}) recover
  strong, well-localised effects on hallucinations
  ($d{=}+0.85$ and $d{=}+0.76$ respectively) by reasoning about the
  chain's internal premise--conclusion link rather than against a sparse
  external source. The same two verdict-link metrics also detect
  omission and contradiction, providing a uniform automatic check across
  all three perturbation types.

==> latex/tables/chain_pert_results.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{llccc}
\toprule
\textbf{Final Judgment} & \textbf{Error Type} & \textbf{Detection (\%)} & \textbf{Agreement (1-7)} & \textbf{Trust (1-7)} \\
\midrule
Correct   & Clean          &  4  & 5.86 & 4.45 \\
          & Omission       & 31  & 5.15 & 3.72 \\
          & Contradiction  & 55  & 4.62 & 3.10 \\
          & Hallucination  & 51  & 4.68 & 3.02 \\
\midrule
Incorrect & Clean          & 27  & 2.54 & 1.97 \\
          & Omission       & 48  & 2.81 & 1.98 \\
          & Contradiction  & 82  & 2.45 & 1.55 \\
          & Hallucination  & 78  & 2.07 & 1.43 \\
\bottomrule
\end{tabular}
\caption{\textbf{Main outcomes across conditions (error type $\times$ correctness).} We observe strong agreement-trust coupling and clear error-type differences, with \emph{omissions} the hardest to detect.}
\label{tab:main_results}
\end{table*}


==> latex/tables/error_profiling_validation.tex <==
\label{sec:model_profiling}
\begin{table}[t]
\centering
\small
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}{lcc}
\toprule
\textbf{Validation Task} & \textbf{Agreement} & \textbf{Cohen’s $\kappa$} \\
\midrule
Error Prevalence Profiling & 92\% & 0.86 \\
Epistemic Tone Profiling & 94\% & 0.89 \\
\bottomrule
\end{tabular}}
\caption{
\textbf{Verification of error and tone profiling.}
Results of two annotators reviewing reasoning chains for both error types and tones evaluated with GPT-4.
}
\label{tab:llm_validation}
\end{table}

==> latex/tables/rq1_calibration_pattern_table.tex <==
\begin{table}[t]
\centering
\small
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{lccc}
\toprule
\textbf{Subset} & \makecell{\textbf{Detection} \\ $\leftrightarrow$ \textbf{Agreement}} & \makecell{\textbf{Detection} \\ $\leftrightarrow$ \textbf{Trust}} & \makecell{\textbf{Agreement} \\ $\leftrightarrow$ \textbf{Trust}} \\
\midrule
Overall   & $\mathbf{-0.29}$ & $\mathbf{-0.45}$ & $\mathbf{+0.82}$ \\ 
\midrule
Correct   & $-0.15$ & $-0.41$ & $+0.72$ \\
Incorrect & $-0.20$ & $-0.42$ & $+0.64$ \\
\bottomrule
\end{tabular}}
\caption{\textbf{Cross-measure correlations by subsets.} 
Negative correlations indicate that higher agreement and trust coincide with reduced error detection. 
% Similar patterns within both \textsc{Correct} and \textsc{Incorrect} subsets suggest that this miscalibration is not solely driven by outcome correctness, but by agreement itself.
}
\label{tab:cross_measures}
\end{table}



% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lccc}
% \toprule
% \textbf{Calibration Pairs} & \textbf{Pearson $r$}\\
% \midrule
% Detection $\leftrightarrow$ Agreement & $-0.91$ \\
% Detection $\leftrightarrow$ Trust     & $-0.89$ \\
% Agreement $\leftrightarrow$ Trust     & $+0.97$ \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Cross-measure correlations.} 
% Pairwise Pearson correlations among detection, agreement, and trust reveal systematic miscalibration: 
% participants’ trust primarily tracks agreement rather than reasoning quality. 
% Negative correlations indicate that higher agreement and trust coincide with reduced error detection.}
% \label{tab:cross_measures}
% \end{table}
